Isolation Forest in Novelty Detection Scenario

Data mining offers a diverse toolbox for extracting meaningful structures from complex datasets, with anomaly detection emerging as a critical subfield particularly in the context of streaming or real-time data. Within anomaly detection, novelty detection focuses on identifying previously unseen patterns after training solely on regular data. While classic algorithms such as One-Class SVM or Local Outlier Factor (LOF) have been widely applied, they often lack interpretability and scalability. In this work, we explore the Half-Space Tree (HST) algorithm, originally proposed for streaming anomaly detection, and propose a novel theoretical modification to adapt it specifically for novelty detection tasks. Our approach is grounded in the idea that anomalies i.e., novelties tend to appear in the higher leaves of the tree, which are less frequently visited by regular instances. We analytically demonstrate the effectiveness of this approach using probabilistic analysis, expected depth (EXD) calculations, and combinatorial reasoning. A comparative analysis of expected depths between our modified HST and the original Isolation Forest highlights that novelty points are significantly more isolated in our approach. This supports the hypothesis that HSTs, with appropriate structural adaptation, can serve as interpretable and efficient novelty detectors. The paper contributes a theoretical foundation and supporting analysis for this adaptation, setting the stage for further application and experimentation.

==> sections/abstract.tex <==
\begin{abstract}
This paper introduces a new approach for novelty detection, which builds upon the foundational principles of the Isolation Forest, more specifically the Half-Space Tree algorithm. The enhanced algorithm is described theoretically, detailing modifications that improve its performance in identifying novel data points. Through comparative analysis, significant differences between the traditional Isolation Forest and this enhanced algorithm are highlighted, showcasing modifications that contribute to increased efficacy. Additionally, this paper provides empirical evidence demonstrating that the enhanced algorithm successfully detects novelty data points, an ability absent in the original Isolation Forest. These findings underscore the potential of the approach presented here to advance the field of anomaly detection by providing a more robust tool for identifying novel occurrences in data sets.
\end{abstract}

==> sections/evaluate_unused.tex <==
Consider a minified example depicted in \ref{fig:example_data}. In this example, two chunks of data are in the top left and bottom right corners, respectively. Then, we selected a specific data point that shares one dimension similar to the first chunk and the other with the second one.

Note that the data have no specific distribution. The point at the bottom left has a value of $P_x = [5,5]$ and is not present for the learning phase.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{figures/example6_experiment.pdf}
\caption{Example figure}
\label{fig:example_data}
\end{figure}



\paragraph{Solution: Original approach}
With the original approach fully unsupervised, we feed the whole input (excluding the $P_x$) to the forest and examine the resulting tree.

First, the trivial binary tree $T_0$ is created (xx), with ranges being the min-max values of input.
By doing the recursive steps, the whole tree is constructed.
Figure \ref{fig:example_noutlier_tree_color} shows the constructed binary tree based on the input data.

The evaluation of $P_x$ is as follows:
\begin{itemize}
    \item In the first step, after randomly selecting the dimension $d=1$ and split point $z$ as in (x) $z = 64.37$, the $P_x$ visits the node $\langle 102.0, 105.0\rangle \times \langle 3.0, 7.0\rangle$
    Note that it is enough for the point to fit only the selected dimension.
    \item In the second step, the point visits the node $\langle 102.0, 105.0\rangle \times \langle 5.0, 7.0\rangle$.
    \item This continues until the final leaf $\langle 102.0, 105.0\rangle \times \langle 5.0, 5.0\rangle$ marked gray in Figure \ref{fig:example_noutlier_tree_color}) is reached. This leaf has a depth of 4.
    
\end{itemize}


If we look at the constructed tree in Figure \ref{fig:example_noutlier_tree_color}, we can see that the resulting leaf is relatively deep, considering the depth of the deepest leaf.






\paragraph{Solution: Novelty approach}

The novelty approach, on the other hand, is a semi-supervised method. We feed the whole input (excluding the $P_x$) to the forest and examine the resulting tree.

First, the trivial binary tree $T_0$ with initial ranges is created (xx).
By doing the recursive steps, the whole tree is constructed.
Figure \ref{fig:example_novelty_tree_color} shows the constructed binary tree based on the input data.

The evaluation of $P_x$ is as follows:
\begin{itemize}
    \item In the first step, since the root node has dimension $d=1$ and split point $z = 54$ assigned during the training phase, the point visits the node $\langle 3.0, 54.0\rangle \times \langle 3.0, 105.0\rangle$
    \item In the second step, the point visits the node $\langle 3.0, 28.5\rangle \times \langle 3.0, 105.0\rangle$.
    \item This continues until the final leaf (marked grey in Figure \ref{fig:example_novelty_tree_color}) is reached. This leaf has a depth of 3.
    
\end{itemize}

==> sections/methods_unused.tex <==
\section{Methods - toto se smaže}
\label{sec:methods}
Traditional approaches for anomaly detection consist of either novelty
detection or outlier detection. Novelty detection is an anomaly
detection mechanism where we search for unusual observations 
discovered due to their differences from the training data. Novelty
detection is a semi-supervised anomaly detection technique, whereas
outlier detection uses unsupervised methods. With novelty detection, the
training data is not polluted by anomalous elements, and we are
interested in detecting whether a new observation is an anomaly. In this context, such points are also called novelties. This is a crucial
distinction. The outlier detection is usually presented with data
containing both anomalies and regular observation; it then uses
mathematical models that try to make a distinction between them. The
novelty detection, on the other hand, is usually presented with data with
little to zero anomalies (the proportion of anomalies in the dataset is
called a contamination), and later, when conferred with an anomalous
observation, it makes a decision.

Consider the following example: Figure \ref{fig:example0} contains random datapoints
arranged in a way they form a cluster-like shape. Say this data is our
regular observations.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{figures/example0_gnu.pdf}
\caption{Example figure}
\label{fig:example0}
\end{figure}

When an unsupervised, outlier detection algorithm tries to analyze such
data, it sees the datapoints as a cluster containing both regular and
anomalous observations. Figure X shows the result of evaluating
classical Isolation Forest on such a dataset.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\textwidth]{figures/example0_5_gnu.pdf}
\caption{Example figure}
\label{fig:example05}
\end{figure}

Figure \ref{fig:example05} shows regular observations \(x\) and anomaly observations \(y\)
marked by Isolation Forest
(\texttt{batch\_size\ 128,\ trees\_count:\ 100,\ zbytek\ default}).
Figure x shows that approx. \(10\%\) of observations are anomalies. This
is not unwanted behaviour in the sense of outlier detection but is false
positive observation in the sense of novelty detection because this
data are regular observations that should be marked so.

Another problem is with the unsupervised separation itself. Consider data polluted by anomalies in close to \(1:1\) ratio. Finding the line
itself is evident. Deciding which observations are anomalies without some domain knowledge, on the other hand, is close to impossible.
